Generalization Bounds via Information Density and Conditional Information Density

We present a general approach, based on exponential inequalities, to derive bounds on the generalization error of randomized learning algorithms. Using this approach, we provide bounds on the average generalization error as well as bounds on its tail probability, for both the PAC-Bayesian and single-draw scenarios. Specifically, for the case of sub-Gaussian loss functions, we obtain novel bounds that depend on the information density between the training data and the output hypothesis. When suitably weakened, these bounds recover many of the information-theoretic bounds available in the literature. We also extend the proposed exponential-inequality approach to the setting recently introduced by Steinke and Zakynthinou (2020), where the learning algorithm depends on a randomly selected subset of the available training data. For this setup, we present bounds for bounded loss functions in terms of the conditional information density between the output hypothesis and the random variable determining the subset choice, given all training data. Through our approach, we recover the average generalization bound presented by Steinke and Zakynthinou (2020) and extend it to the PAC-Bayesian and single-draw scenarios. For the single-draw scenario, we also obtain novel bounds in terms of the conditional $\alpha$-mutual information and the conditional maximal leakage.

==> biography.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{hellstrom.png}}]{Fredrik Hellstr\"om} (S'20) received the B.Sc. and M.Sc. degrees in physics from the University of Gothenburg, Gothenburg, Sweden in 2016 and 2018, respectively. He is currently pursuing the Ph.D. degree in electrical engineering at Chalmers University of Technology, Gothenburg, Sweden. His research interests are in the areas of statistical learning theory and machine learning.
      \end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{durisi.png}}]{Giuseppe Durisi} (S'02--M'06--SM'12) received the Laurea degree \emph{summa cum laude} and the Doctor degree both from Politecnico di Torino, Italy, in 2001 and 2006, respectively.
        From 2002 to 2006, he was with Istituto Superiore Mario Boella, Torino, Italy. From 2006 to 2010 he was a postdoctoral researcher at ETH Zurich, Zurich, Switzerland.
        In 2010, he joined Chalmers University of Technology, Gothenburg, Sweden, where he is now full professor with the Communication Systems Group.
        He is co-director of Chalmers ICT Area of Advance, and of Chalmers AI Research Center.
        Dr. Durisi is a senior member of the IEEE. He is the recipient of the 2013 IEEE ComSoc Best Young Researcher Award for the Europe, Middle East, and Africa Region, and is co-author of a paper that won a “student paper award” at the 2012 International Symposium on Information Theory, and of a paper that won the 2013 IEEE Sweden VT-COM-IT joint chapter best student conference paper award.
        In 2015, he joined the editorial board of the IEEE Transactions on Communications as associate editor.
        From 2011 to 2014, he served as publications editor for the IEEE Transactions on Information Theory.
        His research interests are in the areas of communication and information theory and machine learning.
      \end{IEEEbiography}

==> definitions.tex <==

%% FREDRIK COMMANDS AND NEW COMMANDS AND NOTATION
\newcommand{\RNderiv}{ \log\frac{ \dv P_{W\!Z^n}(w,z^n) }{\dv P_W\!P_{Z^n}(w,z^n)} } 
% Expectation symbol
%\safemath{\opE}{\mathbb{E}}

\newcommand{\trainingdata}{\boldsymbol{Z}}
\newcommand{\trainingdatasmall}{\boldsymbol{z}}
\newcommand{\supersample}{\tilde{\boldsymbol{Z}}}
\newcommand{\supersamplesmall}{\tilde{\boldsymbol{z}}}
\newcommand{\subsetchoice}{\boldsymbol{S}}
\newcommand{\subsetchoiceR}{\boldsymbol{R}}
\newcommand{\subsetchoicesmall}{\boldsymbol{s}}

\newcommand{\genop}{\textnormal{gen}}
\newcommand{\gen}{\genop(W,\trainingdata)}
\newcommand{\genwz}{\genop(w,\trainingdatasmall)}
\newcommand{\genwZ}{\genop(w,\trainingdata)}
\newcommand{\genWz}{\genop(W,\trainingdatasmall)}
\newcommand{\genpertask}{\genop^k}
\newcommand{\genovertasks}{\genop^U}
\newcommand{\genS}{\genop(W,\trainingdata(\subsetchoice))}
\newcommand{\genShat}{\widehat\genop(W,\supersample, \subsetchoice)}
\newcommand{\genShatwz}{\widehat\genop(w,\widetilde{\boldsymbol{z}}, \subsetchoice)}

\newcommand{\jointdistro}{P_{W\! \supersample\! \subsetchoice }}
\newcommand{\pacBdistro}{P_{W\vert \supersample\! \subsetchoice }}

\newcommand{\trainloss}{L_{\trainingdata(\subsetchoice)}(W)}
\newcommand{\trainlossstandard}{L_{\trainingdata}(W)}
\newcommand{\trainlossi}{L_{\trainingdata_i}(W)}
\newcommand{\testloss}{L_{\trainingdata(\bar\subsetchoice)}(W)}
\newcommand{\poploss}{L_{P_Z}(W)}
\newcommand{\poplossw}{L_{P_Z}(w)}
\newcommand{\geniwz}{\widehat{\textnormal{gen}}_i(w,\supersamplesmall, S_i)}
\newcommand{\geniWZ}{\widehat{\textnormal{gen}}_i(W,\supersample, S_i)}
\newcommand{\lRNi}{\log \frac{\dv P_{S_i\vert w\supersamplesmall} }{P_{S_i}} }
\newcommand{\lRNiWZ}{\log \frac{\dv P_{S_i\vert W\!\supersample} }{P_{S_i}} }
\newcommand{\logQRN}{\log\frac{ \dv P_{W\! \supersample\!\subsetchoice}}{ \dv Q_{W\vert \supersample}P_{\supersample\! \subsetchoice}}}
\newcommand{\infdensop}{\imath}
\newcommand{\infdens}{\infdensop(W,\trainingdata)}
\newcommand{\condinfdens}{\infdensop(W,\subsetchoice\vert \supersample)}
\newcommand{\condinfdensi}{\infdensop(W,S_i\vert \supersample)}
\newcommand{\trainlosswz}{L_{\trainingdatasmall(\subsetchoice)}(w)}
\newcommand{\testlosswz}{L_{\trainingdatasmall(\bar\subsetchoice)}(w)}
\newtheorem{remark}{Remark}

